Adaptive and Momentum Methods on Manifolds Through Trivializations

Adaptive methods do not have a direct generalization to manifolds as the adaptive term is not invariant. Momentum methods on manifolds suffer from efficiency problems stemming from the curvature of the manifold. We introduce a framework to generalize adaptive and momentum methods to arbitrary manifolds by noting that for every differentiable manifold, there exists a radially convex open set that covers almost all the manifold. Being radially convex, this set is diffeomorphic to $\mathbb{R}^n$. This gives a natural generalization of any adaptive and momentum-based algorithm to a set that covers almost all the manifold in an arbitrary manifolds. We also show how to extend these methods to the context of gradient descent methods with a retraction. For its implementation, we bring an approximation to the exponential of matrices that needs just of 5 matrix multiplications, making it particularly efficient on GPUs. In practice, we see that this family of algorithms closes the numerical gap created by an incorrect use of momentum and adaptive methods on manifolds. At the same time, we see that the most efficient algorithm of this family is given by simply pulling back the problem to the tangent space at the initial point via the exponential map.

==> sec_impact.tex <==
%! TEX root = main.tex
\section{Broader impact}
Even though it is clear that constrained optimization--and as such, optimization on manifolds---is an essential tool for the Machine Learning and Deep Learning community, we do not foresee any direct impact on society of this particular work. Putting it differently, this work has as much positive or negative impact as the rest of general optimization research.


==> table_per_size.tex <==
\begin{table}[t]
    \centering
\begin{minipage}[b]{0.40\columnwidth}
\caption{Best test accuracy at \mnist{} and \pmnist{}.}
\label{tab:mnist}
\scshape
\small
\begin{tabular}{l c c c}
    \toprule
    Model & n & \mnist & \pmnist \\
    \midrule
    \midrule
    \atriv{}$1$ & $170$ & $98.2$ & $95.1$ \\
    \dtriv{}$\infty$ & $170$ & $98.1$ & $95.0$ \\
    \dtriv{}$1$ & $170$ & $\mathbf{98.3}$ & $\mathbf{95.2}$ \\
    \exprnn & $170$ & $98.0$ & $94.9$ \\
    \scornn & $170$ & $97.2$ & $94.8$ \\
    \scurnn & $116$ & $97.6$ & $94.9$ \\
    \lstm & $128$ & $81.9$ & $79.5$ \\
    \rgd & $116$ & $94.7$ & $92.5$ \\
    \midrule
    \atriv{}$1$ & $360$ &  $\mathbf{98.9}$ & $96.4$ \\
    \dtriv{}$\infty$ & $360$ &  $\mathbf{98.9}$ & $\mathbf{96.5}$ \\
    \dtriv{}$1$ & $360$ &  $98.4$ & $96.3$ \\
    \exprnn & $360$ & $98.4$ & $96.2$ \\
    \scornn & $360$ & $98.1$ & $95.9$ \\
    \scurnn & $250$ & $98.3$ & $96.2$ \\
    \lstm & $256$ & $88.8$ & $88.8$ \\
    \rgd & $256$ & $96.1$ & $93.9$ \\
    \midrule
    \atriv{}$1$ & $512$ & $\mathbf{99.0}$ & $96.7$ \\
    \dtriv{}$\infty$ & $512$ & $\mathbf{99.0}$ & $\mathbf{96.8}$ \\
    \dtriv{}$1$ & $512$ & $98.7$ & $96.7$ \\
    \exprnn & $512$ & $98.7$ & $96.6$ \\
    \scornn & $512$ & $98.2$ & $96.5$ \\
    \lstm & $512$ & $91.9$ & $91.8$ \\
    \rgd & $512$ & $97.3$ & $94.7$ \\
    \bottomrule
\end{tabular}
\end{minipage}
\hspace{0.05\columnwidth}
\begin{minipage}[b]{0.45\columnwidth}
\caption{Test \mse{} at the end of the epoch with the lowest validation \mse{} for the \timit{} task.}
\label{tab:timit}
\small
\scshape
\begin{tabular}{l c c c c}
    \toprule
    Model & n & Val. \mse{} & Test \mse{}\\
    \midrule
    \midrule
    \atriv{}$1$ & $224$ & $\mathbf{4.52}$ & $\mathbf{4.50}$ \\
    \dtriv{}$\infty$ & $224$ & $4.75$ & $4.71$ \\
    \dtriv{}$1$ & $224$ & $6.55$ & $6.54$ \\
    \exprnn & $224$ & $5.34$ & $5.30$ \\
    \scornn & $224$ & $9.26$ & $8.50$ \\
    \scurnn & $128$ & $9.42$ & $7.23$ \\
    \lstm & $84$ &  $15.42$ & $14.30$ \\
    \rgd & $128$ &  $15.07$ & $14.58$ \\
    \midrule
    \atriv{}$1$ & $322$ & $\mathbf{3.33}$ & $\mathbf{3.29}$ \\
    \dtriv{}$\infty$ & $322$ & $3.39$ & $3.76$ \\
    \dtriv{}$1$ & $322$ & $4.56$ & $4.55$ \\
    \exprnn & $322$ & $4.42$ & $4.38$ \\
    \scornn & $322$ & $8.48$ & $7.82$ \\
    \lstm & $120$ & $13.93$ & $12.95$ \\
    \rgd & $192$ & $15.10$ & $14.50$ \\
    \midrule
    \atriv{}$1$ & $425$ & $\mathbf{1.93}$ & $\mathbf{1.92}$ \\
    \dtriv{}$\infty$ & $425$ & $2.00$ & $1.97$ \\
    \dtriv{}$1$ & $425$ & $4.21$ & $4.17$ \\
    \exprnn & $425$ & $5.52$ & $5.48$ \\
    \scornn & $425$ & $7.97$ & $7.36$ \\
    \scurnn & $258$ & $4.40$ & $3.39$ \\
    \lstm & $158$ & $13.66$ & $12.62$ \\
    \rgd & $256$ & $14.96$ & $14.69$ \\
    \bottomrule
\end{tabular}
\end{minipage}
\end{table}

